Randomness extraction and asymptotic Hamming distance

We obtain a non-implication result in the Medvedev degrees by studying sequences that are close to Martin-L\"of random in asymptotic Hamming distance. Our result is that the class of stochastically bi-immune sets is not Medvedev reducible to the class of sets having complex packing dimension 1.

==> figure-table.tex <==
\begin{figure}
	\[
		\xymatrix{
		&
		&
		&
		&
		&
		& 
		&.
		\\
			&
			&
			&
			&
			\color{green}
			\DNC_{2}
				\ar[ddddr]
				\ar@{=>}[dl] &
			& 
			&.
			\\
			\color{red}
			\text{generic}
				\ar[dddddddd]
				\ar[ddr] &
			&
			&
			*+[F]{\text{MLR}}
				\ar[dr]
				\ar[d]
				\ar[dl]
				\ar[dddr] &
			&
			&
			&.
			\\
			&
			&
			*+[F]{\text{SR}}
				\ar[d]
				\ar[dl] &
			*+[F]{\text{KLS}}
				\ar[d]
				\ar^{\text{\cite{MMNRS}}}[dddr] &
			*+[F]{\subseteq\supseteq\text{MLR}}\ar[dll]\ar[ddd] &
			&
			&.
			\\
			&
			*+[F]{\color{red}\text{KR}}
				\ar[dd]
				\ar[ddr]
				\ar@/^/[ddddddddddr] &
			*+[F]{\subseteq\supseteq\text{SR}}
				\ar[ddl]
				\ar[dr] &
			*+[F]{\text{MWC}}
				\ar[d]
				\ar^{\text{\cite{Merkle}}}[ddddddddll] &
			&
			&
			&.
			\\
			&
			&
			&
			*+[F]{\text{SBI}^{2}}
				\ar[d]
				\ar[dl] &
			\text{\tiny pairwiseMLR}
				\ar[dl] &
			\color{green}\DNC_{3}\ar[ddr]
				\ar@{=>}[dl]
				\ar@/_/@{~>}[dlll] &
				&.
			\\
			&
			*+[F]{\color{red}\subseteq\supseteq\text{KR}}
				\ar[ddddddddrrr] &
			*+[F]{\color{red}\text{BI}^{2}}
				\ar[ddddddddrr]	&
			*+[F]{\text{SBI}}\ar[d]
				\ar@{=>}@/^/_{\text{\ref{holdem}}}[dddddddr] &
			*+[F]{H,1}
				\ar[ddd]
				\ar_{\ne}^{\text{\cites{Miller, BDS}}}[dr] &
&
				&.
			\\
			&
			&
			&
			*+[F]{\color{blue}\SDI}
				\ar[dddddddl]
				\ar[dd]
				\ar[dddddddr] &
			&
			*+[F]{H,>0}
				\ar[ddd] &
				\text{DNC}_h&.
			\\
			&
			&
			&
			&
			&
			&\text{aeDNC}_h\ar[dddl]
			&
			\\
			&
			&
&
			*+[F]{\color{blue}\SDI^{-}} &
			*+[F]{cp,1}
				\ar@{~>}_{\text{ \ref{notsur}}}[l]
				\ar[dllll]
				\ar[dr] &
			&
			&.
			\\
			*+[F]{\color{red}p,1}
				\ar_{\ne}^{\text{\cite{Conidis}}}[d] &
			&
			&
			&
			&
			*+[F]{cp,>0}
				\ar^{\text{\ref{cp} (\cite{KMS}); }}[d]
				\ar[dlllll]	
				& \text{COM}_h\ar[ddl]
			\\
			*+[F]{\color{red}p,>0}
				\ar[dr] &
			&
			&
			&
			&\text{COM}
				\ar[dllll]\ar[dddr]
			&
			&
			\\
			&
			*+[F]{\color{red}\neg \text{\tiny WCET}}
				\ar[ddr]
			&
			&
			&						
			&{\color{green}\text{aeDNC}_\text{(REC)}}\ar[dl]\ar[ddl]		
			\\
			&
			&
			&
			&
			\text{ED}
				\ar[drr]
				\ar[dll] 
			&		
			\\
			&
			&
			{\color{red}\neg\text{CT}} &
			&*+[F]{\color{red}\text{BI}} 			
			&& \not\le_{T}\text{generic}			
			&.
			\\
		}		 
	\]
	\caption{
		Some Medvedev degrees.
		See Figures \ref{explain} and \ref{sane} for definitions.
		Colors:
		{\color{red} comeager},
		{\color{blue} not known},
		{measure 1 but meager}. 
	}
	\label{crazy}
\end{figure}



\begin{figure}
	\[
		\xymatrix{
			\ar@{.>}[r] & \text{Muchnik above} \\
			\ar[r] & \text{Included in} \\
			\ar@{~>}[r] & \text{Not Medvedev above} \\
			\ar@{=>}[r] & \text{Medvedev above} \\
		}
	\]
	\caption{Meaning of arrows.}
	\label{explain}
\end{figure}

\begin{figure}
	\begin{tabular}{|c|c|c|}
		\hline
		Abbreviation &
		Unabbreviation &
		Definition \\
		\hline
		\(\DNC\) &
		Diagonally non-recursive function in \(\omega^{\omega}\) &
		\\
		\(\DNC_{n}\) &
		Diagonally non-recursive function in \(n^{\omega}\) &
		\\
		\hline
		\(\MLR\) &
		Martin-L\"of random	&
		\\
		KLR	&
		Kolmogorov-Loveland random	(MLR\(\equiv_{s}\)KLR) &
		\\
		SR &
		Schnorr random &
		\\
		KR &
		Kurtz random (weakly 1-random) &
		\\
		\hline
		\(\MWC\) &
		Mises-Wald-Church stochastic &
		\ref{MWCdef} \\
		KLS	&
		Kolmogorov-Loveland stochastic &
		\ref{KLSdef} \\
		SBI	&
		Stochastically bi-immune &
		\ref{SBIdef} \\
		BI &
		bi-immune &
		\ref{BIdef} \\
		IM &
		immune (equivalently under \(\equiv_{s}\): noncomputable) &
		\ref{BIdef} \\
		\hline
		\((H,1)\)	&
		effective Hausdorff dimension 1	&
		\ref{dimdef} \\
		\((H,>0)\) &
		effective Hausdorff dimension \(>0\) &
		\ref{dimdef} \\
		\((p,1)\)	&
		effective packing dimension 1 &
		\ref{dimdef} \\
		\((p,>0)\) &
		effective packing dimension \(>0\) &
		\ref{dimdef} \\
		\((cp,1)\) &
		complex packing dimension 1	&
		\ref{dimdef} \\
		\((cp,>0)\) &
		complex packing dimension \(>0\) &
		\ref{dimdef} \\
		\hline
		COM	&
		complex in the sense of \cite{KMS} &
		\ref{complexdef} \\
		ED &
		eventually different &
		\ref{EDdef} \\
		\(\not\le_{T}\) Cohen generic	&
		not computable from a 2-generic set &
		\\
		CT &
		computably traceable &
		\\
		WCET &
		weakly c.e.\ traceable &
		\ref{WCETdef} \\
		\hline
	\end{tabular}
	\caption{Abbreviations used in Figure \ref{crazy}.}
	\label{sane}
\end{figure}

